Calibrated Top-1 Uncertainty estimates for classification by score based models

While the accuracy of modern deep learning models has significantly improved in recent years, the ability of these models to generate uncertainty estimates has not progressed to the same degree. Uncertainty methods are designed to provide an estimate of class probabilities when predicting class assignment. While there are a number of proposed methods for estimating uncertainty, they all suffer from a lack of calibration: predicted probabilities can be off from empirical ones by a few percent or more. By restricting the scope of our predictions to only the probability of Top-1 error, we can decrease the calibration error of existing methods to less than one percent. As a result, the scores of the methods also improve significantly over benchmarks.

==> ConCommands.tex <==
%%%%%%%%%%%%%%%%%%%%
% Packages --------------
\usepackage{siunitx}
\sisetup{detect-weight,output-exponent-marker=\ensuremath{\mathrm{e}}}
\usepackage{multirow}



%%%%%%%%%%%%%%%%%%%%
% THEOREM Environments --------------
\theoremstyle{Proposition}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{example}[theorem]{Example}
%%%%%%%%%%%%%%%%%%%%
%----------------------------------------------
%% Basic Commands
\DeclareMathOperator{\argmin}{{argmin}}
%\DeclareMathOperator{\argmax}{{argmax}}
\DeclareMathOperator{\sgn}{{sgn}}
\DeclareMathOperator{\dist}{{dist}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rd}{\R^d}
\newcommand{\Rn}{\R^n}
\newcommand{\e}{\epsilon}
\newcommand{\bO}{\mathcal{O}}
\newcommand{\E}[1]{\mathbb{E} \left [{#1}\right ]}
%\DeclareMathOperator{\mb}{mb}
\newcommand{\mb}{{b}}

\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\norm}[1]{\left|#1\right|}


==> paper-commands.tex <==
\usepackage{tikz}
\usepackage{url}
%----------------------------------------------

\usepackage{color}
\usepackage{graphicx}
\usepackage{float}
%\usepackage{subcaption}
\usepackage{multirow}
\usepackage{siunitx}
\sisetup{detect-weight,output-exponent-marker=\ensuremath{\mathrm{e}}}
%%%%%%%%%%%%%%%%%%%%



% THEOREM Environments --------------
\theoremstyle{Proposition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{principle}{Principle}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{method}[theorem]{Method}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}


%%%%%%%%%%%%%%%%%%%%
%  Basic Commands
%%%%%%%%%%%%%%%%%%%%
%----------------------------------------------
% norms, absolute value
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\Norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\vert#1\vert}
\newcommand{\Abs}[1]{\left\vert#1\right\vert}

%% Basic Commands
\DeclareMathOperator{\grad}{\nabla}
\DeclareMathOperator{\diag}{{diag}}
\DeclareMathOperator{\softmax}{{softmax}}
\DeclareMathOperator{\KL}{{KL}}
\DeclareMathOperator{\Lp}{Lip}
\DeclareMathOperator*{\argmin}{{arg\,min}}
\DeclareMathOperator*{\argmax}{{arg\,max}}
\DeclareMathOperator{\sgn}{{sgn}}
\DeclareMathOperator{\dist}{{dist}}


\newcommand{\R}{\mathbb{R}}

\newcommand{\Rd}{\R^d}
\newcommand{\Rn}{\R^n}
\newcommand{\e}{\varepsilon}
\newcommand{\bO}{\mathcal{O}}
\newcommand{\Lip}{Lipschitz}

%% Sectioning Commands
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}



\newcommand{\loss}{\mathcal{L}}
\newcommand{\lossN}[1]{\loss_{\rm{#1}}}
\newcommand{\LD}{L_{\mathcal D}}
\newcommand{\fC}{\mathbf{y}}
\newcommand{\fCC}[1]{\fC_{\rm{#1}}}
\newcommand{\fM}{f}

\newcommand{\PP}{\mathbb{P}} 
\newcommand{\DataSupp}{\mathcal{X}}
\newcommand{\DS}{S}
\newcommand{\DSS}[1]{{\DS}^{\rm{#1}}}
\newcommand{\pdata}{\PP_{\rm{data}}}
\newcommand{\pdataT}[1]{\pdata^{\rm{#1}}}
%\newcommand{\pdataN}{p_{\rm{data}}^{\rm{train}}}

\newcommand{\YY}{\mathcal{Y}}
\newcommand{\cc}{{c}}
\newcommand{\Functions}{\mathcal{F}}
%\newcommand{\pdataTest}{\widehat{p}_{\rm{data}}^{\rm{test}}}
\newcommand{\ClassProject}{\mathbf{\pi}}
\newcommand{\Err}{\epsilon}
\newcommand{\ErrTT}[2]{\Err_{{#1}}^{\rm{#2}}}
\newcommand{\EE}{\mathbb{E}}
% Probability
\newcommand{\EEE}[1]{{\mathbb{E}}^{\rm{#1}}}
\newcommand{\gap}{\Err^{\rm{gap}}}
\newcommand{\ee}[1]{\mathbf{e}^{(#1)}}
%\newcommand{\ErrT}[1]{\epsilon^}

\newcommand{\Reg}{\mathcal R}


